Simple closed geodesics on most Alexandrov surfaces

We study the existence of simple closed geodesics on most (in the sense of Baire category) Alexandrov surfaces with curvature bounded below, compact and without boundary. We show that it depends on both the curvature bound and the topology of the surfaces.

==> Macros.tex <==

\newcommand{\nc}{\newcommand}
\newcommand{\df}{\def}
\RequirePackage{ifthen}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%racourciss divers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\df\ie#1{{\it \mbox{i.\hspace{0.06em}e.\ifthenelse{\equal{#1}{,}}{\hspace{0.06em},}{\ #1}}}}
\df\eg#1{{\it \mbox{e.\hspace{0.06em}g.\ifthenelse{\equal{#1}{,}}{\hspace{0.06em},}{\ #1}}}}

%%%%%%%%%TURNED-M
\newcommand{\most}{\raisebox{-.05em}{\rotatebox[origin=c]{180}{\ensuremath{\mathsf{M}}}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Citations dans Theorem
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\cit}[2][]{\ifthenelse{\equal{#1}{}}{{\rm \cite{#2}}}{{\rm \cite[#1]{#2}}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Gestions des {|}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% usage:
% \set(:bla ... | blajjxo..:) (in display)
% \set[2](: | :) (if nested sets, gives the nesting degree, up to 4)
% \seti(: | :)  or \seti[2](: | :) (outside display (i=inline))


\makeatletter
\newlength{\JR@setLa}
\newlength{\JR@setLb}
\newlength{\JR@setLc}
\newlength{\JR@setLd}
\newlength{\JR@setLe}
\nc{\JR@setMta}{}
\nc{\JR@setMtb}{}
\nc{\JR@setMtc}{}
\nc{\JR@setMtd}{}

\nc{\JR@setMt}[1]{
\ifthenelse{#1=1}{\JR@setMta}{}
\ifthenelse{#1=2}{\JR@setMtb}{}
\ifthenelse{#1=3}{\JR@setMtc}{}
\ifthenelse{#1=4}{\JR@setMtd}{}
}


\nc{\JR@max}[3]{\ifthenelse{\lengthtest{\the#1>\the#2}}
           {\setlength{#3}{#1}}
           {\setlength{#3}{#2}}}


\nc{\JR@setds}{}
\nc{\JR@setSD}[4][]{
 \ifthenelse{\equal{#1}{}}
   {\renewcommand{\JR@setds}{}}
   {\renewcommand{\JR@setds}{\displaystyle}}
 \settoheight{\JR@setLa}{\ensuremath{\JR@setds{#2}}}
 \settoheight{\JR@setLb}{\ensuremath{\JR@setds{#3}}}
 \settodepth{\JR@setLc}{\ensuremath{\JR@setds{#2}}}
 \settodepth{\JR@setLd}{\ensuremath{\JR@setds{#3}}}
 \settowidth{\JR@setLe}{\ensuremath{\JR@setds{\left.\right.}}}
 \JR@max{\JR@setLc}{\JR@setLd}{\JR@setLc}
 \JR@max{\JR@setLa}{\JR@setLb}{\JR@setLa}
 \addtolength{\JR@setLa}{\JR@setLc}
 \ifthenelse{#4=1}{\renewcommand{\JR@setMta}{\rule[-\JR@setLc]{0pt}{\JR@setLa}}}{}
 \ifthenelse{#4=2}{\renewcommand{\JR@setMtb}{\rule[-\JR@setLc]{0pt}{\JR@setLa}}}{}
 \ifthenelse{#4=3}{\renewcommand{\JR@setMtc}{\rule[-\JR@setLc]{0pt}{\JR@setLa}}}{}
 \ifthenelse{#4=4}{\renewcommand{\JR@setMtd}{\rule[-\JR@setLc]{0pt}{\JR@setLa}}}{}
} 
 

\df\SetEx[#1,#2](:#3|#4:){
 \JR@setSD[#2]{#3}{#4}{#1}
 \left\{\JR@setMt{#1} #3\right.\left|\rule{.9\JR@setLe}{0pt}#4 \JR@setMt{#1}\right\}
}


\nc{\set}[1][1]{\SetEx[#1,ds]}
\nc{\seti}[1][1]{\SetEx[#1,]}



\makeatother


